Reliable Real Time Ball Tracking for Robot Table Tennis

Robot table tennis systems require a vision system that can track the ball position with low latency and high sampling rate. Altering the ball to simplify the tracking using for instance infrared coating changes the physics of the ball trajectory. As a result, table tennis systems use custom tracking systems to track the ball based on heuristic algorithms respecting the real time constrains applied to RGB images captured with a set of cameras. However, these heuristic algorithms often report erroneous ball positions, and the table tennis policies typically need to incorporate additional heuristics to detect and possibly correct outliers. In this paper, we propose a vision system for object detection and tracking that focus on reliability while providing real time performance. Our assumption is that by using multiple cameras, we can find and discard the errors obtained in the object detection phase by checking for consistency with the positions reported by other cameras. We provide an open source implementation of the proposed tracking system to simplify future research in robot table tennis or related tracking applications with strong real time requirements. We evaluate the proposed system thoroughly in simulation and in the real system, outperforming previous work. Furthermore, we show that the accuracy and robustness of the proposed system increases as more cameras are added. Finally, we evaluate the table tennis playing performance of an existing method in the real robot using the proposed vision system. We measure a slight increase in performance compared to a previous vision system even after removing all the heuristics previously present to filter out erroneous ball observations.

==> fig/success.tex <==
% This file was created by matplotlib2tikz v0.6.14.
\begin{tikzpicture}

\begin{axis}[
xlabel={Success rate \%},
ylabel={Probability},
xmin=-5, xmax=105,
ymin=0, ymax=0.25,
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black},
legend style={draw=white!80.0!black},
legend cell align={left},
legend entries={{ProMP Old},{ProMP New}}
]
\addlegendimage{ybar,fill=red,draw opacity=0,fill opacity=0.2,area legend};
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:0,0) rectangle (axis cs:2.04081632653061,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:2.04081632653061,0) rectangle (axis cs:4.08163265306123,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:4.08163265306122,0) rectangle (axis cs:6.12244897959184,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:6.12244897959184,0) rectangle (axis cs:8.16326530612245,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:8.16326530612245,0) rectangle (axis cs:10.2040816326531,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:10.2040816326531,0) rectangle (axis cs:12.2448979591837,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:12.2448979591837,0) rectangle (axis cs:14.2857142857143,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:14.2857142857143,0) rectangle (axis cs:16.3265306122449,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:16.3265306122449,0) rectangle (axis cs:18.3673469387755,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:18.3673469387755,0) rectangle (axis cs:20.4081632653061,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:20.4081632653061,0) rectangle (axis cs:22.4489795918367,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:22.4489795918367,0) rectangle (axis cs:24.4897959183673,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:24.4897959183673,0) rectangle (axis cs:26.530612244898,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:26.530612244898,0) rectangle (axis cs:28.5714285714286,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:28.5714285714286,0) rectangle (axis cs:30.6122448979592,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:30.6122448979592,0) rectangle (axis cs:32.6530612244898,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:32.6530612244898,0) rectangle (axis cs:34.6938775510204,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:34.6938775510204,0) rectangle (axis cs:36.734693877551,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:36.734693877551,0) rectangle (axis cs:38.7755102040816,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:38.7755102040816,0) rectangle (axis cs:40.8163265306123,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:40.8163265306122,0) rectangle (axis cs:42.8571428571429,0.0002);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:42.8571428571429,0) rectangle (axis cs:44.8979591836735,0.0006);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:44.8979591836735,0) rectangle (axis cs:46.9387755102041,0.001);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:46.9387755102041,0) rectangle (axis cs:48.9795918367347,0.004);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:48.9795918367347,0) rectangle (axis cs:51.0204081632653,0.0052);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:51.0204081632653,0) rectangle (axis cs:53.0612244897959,0.0136);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:53.0612244897959,0) rectangle (axis cs:55.1020408163265,0.0245999999999999);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:55.1020408163265,0) rectangle (axis cs:57.1428571428571,0.0354000000000006);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:57.1428571428572,0) rectangle (axis cs:59.1836734693878,0.0538000000000015);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:59.1836734693878,0) rectangle (axis cs:61.2244897959184,0.0768000000000022);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:61.2244897959184,0) rectangle (axis cs:63.265306122449,0.0943999999999944);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:63.265306122449,0) rectangle (axis cs:65.3061224489796,0.108999999999988);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:65.3061224489796,0) rectangle (axis cs:67.3469387755102,0.112599999999988);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:67.3469387755102,0) rectangle (axis cs:69.3877551020408,0.119399999999987);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:69.3877551020408,0) rectangle (axis cs:71.4285714285714,0.100399999999989);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:71.4285714285714,0) rectangle (axis cs:73.4693877551021,0.0865999999999905);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:73.469387755102,0) rectangle (axis cs:75.5102040816327,0.0655999999999928);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:75.5102040816327,0) rectangle (axis cs:77.5510204081633,0.0429999999999953);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:77.5510204081633,0) rectangle (axis cs:79.5918367346939,0.0261999999999971);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:79.5918367346939,0) rectangle (axis cs:81.6326530612245,0.0145999999999984);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:81.6326530612245,0) rectangle (axis cs:83.6734693877551,0.00799999999999912);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:83.6734693877551,0) rectangle (axis cs:85.7142857142857,0.00319999999999965);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:85.7142857142857,0) rectangle (axis cs:87.7551020408163,0.00159999999999982);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:87.7551020408163,0) rectangle (axis cs:89.7959183673469,0.000199999999999978);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:89.795918367347,0) rectangle (axis cs:91.8367346938776,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:91.8367346938776,0) rectangle (axis cs:93.8775510204082,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:93.8775510204082,0) rectangle (axis cs:95.9183673469388,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:95.9183673469388,0) rectangle (axis cs:97.9591836734694,0);
\draw[fill=red,draw opacity=0,fill opacity=0.2] (axis cs:97.9591836734694,0) rectangle (axis cs:100,0);

\addlegendimage{ybar,fill=green,draw opacity=0,fill opacity=0.2,area legend};
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:0,0) rectangle (axis cs:2.04081632653061,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:2.04081632653061,0) rectangle (axis cs:4.08163265306123,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:4.08163265306122,0) rectangle (axis cs:6.12244897959184,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:6.12244897959184,0) rectangle (axis cs:8.16326530612245,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:8.16326530612245,0) rectangle (axis cs:10.2040816326531,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:10.2040816326531,0) rectangle (axis cs:12.2448979591837,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:12.2448979591837,0) rectangle (axis cs:14.2857142857143,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:14.2857142857143,0) rectangle (axis cs:16.3265306122449,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:16.3265306122449,0) rectangle (axis cs:18.3673469387755,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:18.3673469387755,0) rectangle (axis cs:20.4081632653061,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:20.4081632653061,0) rectangle (axis cs:22.4489795918367,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:22.4489795918367,0) rectangle (axis cs:24.4897959183673,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:24.4897959183673,0) rectangle (axis cs:26.530612244898,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:26.530612244898,0) rectangle (axis cs:28.5714285714286,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:28.5714285714286,0) rectangle (axis cs:30.6122448979592,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:30.6122448979592,0) rectangle (axis cs:32.6530612244898,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:32.6530612244898,0) rectangle (axis cs:34.6938775510204,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:34.6938775510204,0) rectangle (axis cs:36.734693877551,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:36.734693877551,0) rectangle (axis cs:38.7755102040816,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:38.7755102040816,0) rectangle (axis cs:40.8163265306123,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:40.8163265306122,0) rectangle (axis cs:42.8571428571429,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:42.8571428571429,0) rectangle (axis cs:44.8979591836735,0.0002);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:44.8979591836735,0) rectangle (axis cs:46.9387755102041,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:46.9387755102041,0) rectangle (axis cs:48.9795918367347,0.0008);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:48.9795918367347,0) rectangle (axis cs:51.0204081632653,0.0022);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:51.0204081632653,0) rectangle (axis cs:53.0612244897959,0.0034);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:53.0612244897959,0) rectangle (axis cs:55.1020408163265,0.00840000000000002);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:55.1020408163265,0) rectangle (axis cs:57.1428571428571,0.0167999999999999);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:57.1428571428572,0) rectangle (axis cs:59.1836734693878,0.0237999999999999);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:59.1836734693878,0) rectangle (axis cs:61.2244897959184,0.0476000000000011);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:61.2244897959184,0) rectangle (axis cs:63.265306122449,0.0622000000000018);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:63.265306122449,0) rectangle (axis cs:65.3061224489796,0.0832000000000024);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:65.3061224489796,0) rectangle (axis cs:67.3469387755102,0.0997999999999892);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:67.3469387755102,0) rectangle (axis cs:69.3877551020408,0.120599999999987);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:69.3877551020408,0) rectangle (axis cs:71.4285714285714,0.123199999999986);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:71.4285714285714,0) rectangle (axis cs:73.4693877551021,0.113399999999988);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:73.469387755102,0) rectangle (axis cs:75.5102040816327,0.099599999999989);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:75.5102040816327,0) rectangle (axis cs:77.5510204081633,0.0791999999999913);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:77.5510204081633,0) rectangle (axis cs:79.5918367346939,0.054399999999994);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:79.5918367346939,0) rectangle (axis cs:81.6326530612245,0.0323999999999964);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:81.6326530612245,0) rectangle (axis cs:83.6734693877551,0.0163999999999982);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:83.6734693877551,0) rectangle (axis cs:85.7142857142857,0.00779999999999914);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:85.7142857142857,0) rectangle (axis cs:87.7551020408163,0.0035999999999996);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:87.7551020408163,0) rectangle (axis cs:89.7959183673469,0.000599999999999934);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:89.795918367347,0) rectangle (axis cs:91.8367346938776,0.000199999999999978);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:91.8367346938776,0) rectangle (axis cs:93.8775510204082,0.000199999999999978);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:93.8775510204082,0) rectangle (axis cs:95.9183673469388,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:95.9183673469388,0) rectangle (axis cs:97.9591836734694,0);
\draw[fill=green,draw opacity=0,fill opacity=0.2] (axis cs:97.9591836734694,0) rectangle (axis cs:100,0);
\end{axis}

\end{tikzpicture}


==> sections/appendices.tex <==

\section{Appendix if needed}



\begin{comment}
\section{Appendix Title Goes Here}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...
\end{comment}



==> sections/removed.tex <==

\subsection{Object Detection}

\begin{itemize}
  \item In this section we evaluate different alternatives to detect the table tennis
    ball in an image and possibly some other objects of interest
  \item First, we record images with the ball attached to the robot and the corresponding
    ball positions. We use the same set of images with different detection methods and
    different image resolutions. On each experiment, we measure the accuracy of the
    detected ball position and the running time. We expect to see a tradeoff between accuracy
    and running time by changing both the detection techniques and the image resolution.
  \item We could potentially measure how different approaches require more or less data and
    training time and how it affects the performance.
\end{itemize}

\subsection{Testing the ball model}

\begin{itemize}
  \item Many of the table tennis papers focus a lot on the ball model, but in my opinion
    the evaluation of these models is rather poor.
  \item \cite{mag3} assumes a second order polynomial to be enough to model the ball trajectory.
    But in the evaluation it doesn't seem they test the prediction performance.
  \item In~\cite{chen2015robust}, they use differential equations to model the physics of the
    ball. The constants seem to be taken from other uncited source (model not learned). The
    initial conditions are found fitting a polynomial. To evaluate their prediction, they
    use ball observations of a segment of the trajectory they call \textit{trj-a} and test
    on the rest of the trajectory. However, they do not define clearly these segmentation
    and in the evaluation it is not clear how it predicts in general. They just took one
    single trajectory and plotted the error with respect to time. That seems to be around
    5 cm in each coordinate.
  \item A better way to measure the ball model accuracy could be: Given a particular number
    of observations predict what happens with the rest of the trajectory for multiple instances
    and compute an error distribution. This could be already interesting to show for some
    particular number in the paper. But we could go beyond by computing some statistics like 
    maximum error, average error, ..., and compare for different number of given observations.
  \item On this paper, we evaluate the prediction performance of some of the ball model 
    ideas proposed in previous work as well as some other methods proposed in this paper.
\end{itemize}

\subsubsection{Using a Physical Model}

A recurrent pattern in all the previous work in table tennis is to use known
physical models to predict the ball trajectory. Let~$\vect{x}$ be the position of
the ball, the differential equation used to model the flying behavior of the
ball is given by
%
\[ \vect{\ddot{x}} = \vect{g} - \beta_0|\vect{\dot{x}}|\vect{\dot{x}} - \beta_1 \vect{\omega}_s \times \vect{\dot{x}}, \]
%
where~$\vect{g}$ represents the gravity and~$\vect{\omega}_s$ represents the spin 
of the ball. The constants~$\beta_0$ and~$\beta_1$ represent how much the air drag
and spin forces affect the trajectory of the ball, and depend on several parameters
such as the radius and mass of the ball, density of the air, etc. In~\cite{chen2015robust},
the values provided for~$\beta_0$ and~$\beta_1$ are 0.15 and 0.012 respectively.
Estimating the spin~$\vect{\omega}_s$ is hard. Therefore, the spin is typically
ignored~\cite{mulling2011biomimetic,mag3} or assumed to be constant~\cite{chen2015robust}.
Both of these assumptions are reasonable for
robot table tennis, since the spin given by robots hitting the ball is often 
negligible. For this paper, we decided to ignore the effect of the spin.

\begin{table}
  \centering
  \begin{tabular}{@{}c|cccc@{}}
    \toprule
     & \multicolumn{4}{c}{\bf{Observations}} \\
    \bf{Order} & 12 & 25 & 50 & 75 \\
    \midrule
    2 & 7.17 & 2.77 & \bf{1.51} & 2.06 \\
    3 & 16.16 & 6.05 & 2.52 & 1.76 \\
    4 & 29.02 & 11.12 & 4.49 & 2.92 \\
    \bottomrule
  \end{tabular}
  \caption{
    Average ball trajectory prediction error in centimeters in simulation, using polynomial of
    different orders and different number of observations. The simulated trajectories are generated with
    the same differential equation used for predictions. Therefore, the only source
    of error is how accurate can we estimate the initial position and velocity using
    noisy observations. 
  }
  \label{tab:sim_traj:error}
\end{table}

In addition to the differential equation, we need to estimate the initial position and 
velocity of a ball trajectory given noisy observations. The answer provided in
previous work is to fit a polynomial to a subset of the observations in order to
estimate the initial conditions. The order of the polynomials used range from
second order~\cite{mag3} to fourth order~\cite{chen2015robust}. The number of
observations used to estimate the polynomials is usually not provided.
Table~\ref{tab:sim_traj:error} displays the average prediction error of
simulated trajectories in centimeters using polynomial of different orders and
several number of noisy ball observations to estimate the initial conditions.
For this experiment, the differential
equation used to generate the simulated trajectories and to make the
predictions is exactly the same. Therefore, the source of the error is only
the accuracy of the estimation of the initial state.
Note that the higher the order of the polynomial, the more ball observations
are needed to achieve a similar prediction accuracy. We achieved
the best results, of 1.51 cm average error, using always the last 50 ball 
observations before the bounce with second order polynomials to 
estimate the initial ball position and velocity.


